Universal guarantees for decision tree induction via a higher-order splitting criterion

We propose a simple extension of top-down decision tree learning heuristics such as ID3, C4.5, and CART. Our algorithm achieves provable guarantees for all target functions $f: \{-1,1\}^n \to \{-1,1\}$ with respect to the uniform distribution, circumventing impossibility results showing that existing heuristics fare poorly even for simple target functions. The crux of our extension is a new splitting criterion that takes into account the correlations between $f$ and small subsets of its attributes. The splitting criteria of existing heuristics (e.g. Gini impurity and information gain), in contrast, are based solely on the correlations between $f$ and its individual attributes. Our algorithm satisfies the following guarantee: for all target functions $f : \{-1,1\}^n \to \{-1,1\}$, sizes $s\in \mathbb{N}$, and error parameters $\epsilon$, it constructs a decision tree of size $s^{\tilde{O}((\log s)^2/\epsilon^2)}$ that achieves error $\le O(\mathsf{opt}_s) + \epsilon$, where $\mathsf{opt}_s$ denotes the error of the optimal size $s$ decision tree. A key technical notion that drives our analysis is the noise stability of $f$, a well-studied smoothness measure.

==> DecisionTreesAgnostic.tex <==
%!TEX root = noisy.tex
\section{Universal guarantees}

In this section, we will provide guarantees on the performance of our algorithm for arbitrary function $f: \{0,1\}^n \rightarrow \{0,1\}$. The quality of our guarantees will be dependent on $\opt_s$, where the user can choose the $s$ that leads to the best guarentee. We first need the following proposition.

\begin{proposition}
    \label{prop: agnostic noise sensitivity}
    For any functions $f, g :\pmo^n \to \pmo^n$
    \begin{align*}
        \NS_\delta(g) \leq \NS_\delta(f) + 2 \cdot \Pr_{\bx \in \pmo^n}[f(\bx) \ne g(\bx)].
    \end{align*}
\end{proposition}
\begin{proof}
     We use $\bx \sim \pmo^n$ to denote a uniform random variable and $\by$ a $\delta$-noisy copy of $\bx$.
    \begin{align*}
        \NS_\delta(g) &= \Pr[g(\bx) \neq g(\by)] \\
        &\leq \Pr\bigg[\big(f(\bx) \neq f(\by)\big) \text{ or } \big(f(\bx) \neq g(\bx)\big) \text{ or } \big(f(\by) \neq g(\by)\big)\bigg]\\
        &\leq \Pr[f(\bx) \neq f(\by)] + \Pr[f(\bx) \neq g(\bx)]  + \Pr[f(\by) \neq g(\by)] \tag*{union bound}\\
        &\leq \Pr[f(\bx) \neq f(\by)] + 2 \cdot \Pr[f(\bx) \neq g(\bx)]  \tag*{$\bx$ and $\by$ distributed identically} \\
        &\leq \NS_\delta(f) + 2 \cdot \Pr[f(\bx) \ne g(\bx)] 
    \end{align*} 
\end{proof}

We probably don't need to include this lower bound in the paper, but writing it for us. The $2$ in \Cref{prop: agnostic noise sensitivity} is tight. Let $f$ be the function that is $0$ everywhere and $g$ be $1$ at a single input, $\alpha$, and $0$ everywhere else. Then $\NS_\delta(f) = 0$ and
\begin{align*}
    \NS_\delta(g) &= \Pr[g(\bx) \neq g(\by)]  \\
    &= \Pr[(\bx = \alpha,\by \neq \alpha) \text{ or }(\bx \neq \alpha,\by = \alpha) ] \\
    &\leq \Pr[(\bx = \alpha,\by \neq \alpha)] + \Pr[\bx \neq \alpha,\by = \alpha] \tag*{union bound} \\
    &\leq 2 \cdot \Pr[(\bx = \alpha,\by \neq \alpha)] \tag*{tuples $(\bx,\by)$ and $(\by,\bx)$ identically distributed} \\
    &= 2 \cdot \Pr[\bx = \alpha] \Pr[\by \neq \alpha | \bx = \alpha] \\
    &= 2 \cdot (\frac{1}{2^n}) \cdot (1 - (1 - \eta)^n)\\
    &= 2 \cdot (1 - (1 - \eta)^n) \cdot \Pr[f(\bx) \ne g(\bx)]
\end{align*}
The factor $(1 - (1 - \eta)^n)$ can be arbitrarily close to $1$, proving that \Cref{prop: agnostic noise sensitivity} is tight.

We also need the following facts \textbf{todo, cite}
\begin{fact}
    \label{fact: noise sensitivity from influence}
    For any function $f:\pmo^n \to \pmo$ and $\delta \in [0,1]$
    \begin{align*}
        \NS_\delta(f) \leq \delta \cdot \Inf(f).
    \end{align*}
\end{fact}
\begin{fact}
    \label{fact: influence decision tree}
    For any size-$s$ decision tree $f:\pmo^n \to \pmo$
    \begin{align*}
        \Inf(f) \leq \log(s).
    \end{align*}
\end{fact}
\begin{fact}
    \label{fact: influence monotone decision tree}
    For any size-$s$ monotone decision tree $f:\pmo^n \to \pmo$
    \begin{align*}
        \Inf(f) \leq \sqrt{\log(s)}.
    \end{align*}
\end{fact}

We now prove our universal results.

\textbf{Make align with intro}
\begin{corollary}[Universal guarantee] 
Let $f : \pmo^n \to \zo$ be any function.  For all $s\in \N$ and $\eps \in (0,\frac1{2})$, for $\delta = \frac{\varepsilon}{2 \cdot \log(s)}$ and 
\[ t = s^{O((\log s)/\eps^2)}, \] 
$\BuildStabilizingDT(f,\delta,\frac{\eps}{2},t)$ runs in time $(n+s)^{O(\log(s)/\eps^2)}$ and returns a tree $T$ satisfying $\error_f(T) \le \opt_s +\eps$.  
\end{corollary} 
\begin{proof}
    Let $g$ be the size-$s$ decision tree that is $\opt_s$ close to $f$. Then, 
    \begin{align*}
        \NS_\delta(f) &\leq \NS_\delta(g) + 2 \cdot \opt_s \tag*{\Cref{prop: agnostic noise sensitivity}} \\
        &\leq \delta \cdot \Inf(g)+ 2 \cdot \opt_s \tag*{\Cref{fact: noise sensitivity from influence}} \\
        &\leq \delta \cdot \log(s) + 2 \cdot \opt_s \tag*{\Cref{fact: influence decision tree}} \\
        &\leq \frac{\eps}{2} + 2 \cdot \opt_s \tag*{$\delta = \frac{\varepsilon}{2 \cdot \log(s)}$} 
    \end{align*}
    Plugging the noise stability of $f$ into \Cref{thm:main} gives the desired result. 
\end{proof}

\begin{corollary}[Universal guarantee for Monotone functions] 
Let $f : \pmo^n \to \zo$ be any monotone function.  For all $s\in \N$ and $\eps \in (0,\frac1{2})$, for $\delta = \frac{\varepsilon}{2 \cdot \sqrt{\log(s)}}$ and 
\[ t = s^{O(\sqrt{\log s}/\eps^2)}, \] 
$\BuildStabilizingDT(f,\delta,\frac{\eps}{2},t)$ runs in time $(n+s)^{O(\sqrt{\log(s)}/\eps^2)}$ and returns a tree $T$ satisfying $\error_f(T) \le \opt_s +\eps$.  
\end{corollary} 




==> extra.tex <==
\begin{definition}[$\delta$-noisy influence] 
The {\sl $\delta$-noisy influence of $i$ on $f$} is the quantity 
\[
 \Inf^{(1-2\delta)}_i(f) \coloneqq \Stab_{1-2\delta}[D_i(f)]  = \E\big[D_if(\bx) D_if(\by)\big].
 \] 
\end{definition} 
There's a nice Fourier formula for this quantity: 
\begin{equation}  \Inf_i^{(1-2\delta)}(f) = \sum_{S \ni i} (1-2\delta)^{|S|-1} \wh{f}(S)^2.  \label{eq:noisy-inf-fourier} 
 \end{equation} 
 Note that the ``$0$-noisy influence" of $i$ on $f$ is simply $\Inf_i(f)$. 

\begin{corollary}[Every small-depth DT has a variable of large noisy influence]
\label{cor:noisy-OSSS}
Let $f : \pmo^n \to \pmo$ be computable a size-$s$ decision tree.  Then there is an $i\in [n]$ such that 
\[ \Inf^{(1-2\delta)}_i(f) \ge \frac1{(1-2\delta)^3}\cdot  \frac{\Var(f_\delta)}{\log s} \ge \frac{\Var(f_\delta)}{\log s}.\] 
\end{corollary} 

Consequently, as long as $\Var(f_\delta) \ge \eps$, we are guaranteed the existence of a variable with $\delta$-noisy influence at least 
\[ \Inf_i^{(1-2\delta)}(f) \ge \frac{\eps}{\log s}.\] 
\begin{proof}[Proof of~\Cref{cor:noisy-OSSS}]
Applying~\Cref{thm:OSSS} with $T$ being the size-$s$ DT that computes $f$, and $g$ being $f_\delta$, we get that 
\begin{equation} \Cov(f,f_\delta) \le \sum_{i=1}^n \delta_i(T) \cdot \Inf_i(f_\delta) \le  \max_{i\in [n]}\Big\{ \Inf_i(f_\delta)\Big\}\cdot \log s. \label{eq:apply-OSSS}
\end{equation} 
Next note that the LHS can be lower bounded by:
\begin{align*}  \Cov(f,f_\delta) &= \sum_{S\ne \emptyset} (1-2\delta)^{|S|} \wh{f}(S)^2  \tag*{(Fourier expansion of $f_\delta$ (\ref{eq:smooth-fourier}) and formula for covariance (\ref{eq:covariance}))}\\
&\ge \frac1{1-2\delta}\cdot  \sum_{S\ne \emptyset} (1-2\delta)^{2|S|}\wh{f}(S)^2 \tag*{(since $(1-2\delta)^{2k} \le (1-2\delta)^{k+1}$ for all $k\ge 1$)}  \\
&= \frac{1}{1-2\delta} \cdot \Var(f_\delta).  \tag*{(Formula for variance (\ref{eq:covariance}))}
\end{align*} 
On the other hand, we also have that 
\begin{align*}
 \Inf_i(f_\delta) &= \sum_{S \ni i} (1-2\delta)^{2|S|} \wh{f}(S)^2  \tag*{(Formula for influence (\ref{eq:influence}))} \\
 &\le (1-2\delta)^2 \cdot \sum_{S \ni i} (1-2\delta)^{|S|-1} \wh{f}(S)^2 \tag*{(since $(1-2\delta)^{2k} \le (1-2\delta)^{k+1}$ for all $k\ge 1$)}  \\
 &= (1-2\delta)^2 \cdot \Inf^{(1-2\delta)}_i(f).  \tag*{(Formula for $\delta$-noisy influence (\ref{eq:noisy-inf-fourier}))}
 \end{align*} 
 These two inequalities along with~\Cref{eq:apply-OSSS} give us 
 \[ \frac1{1-2\delta}\cdot \Var(f_\delta) \le \max_{i\in [n]}\Big\{ \Inf_i^{(1-2\delta)}(f)\Big\} \cdot (1-2\delta)^2 \cdot \log s. \] 
 Rearranging completes the proof. 
\end{proof} 

\section{The decision tree for noise stable functions} 

Suppose $f : \pmo^n \to \pmo$ is such that $\NS_\delta(f) \le \kappa$. Consider the partial decision tree $T^\circ$ (with unlabeled leaves) obtained by iteratively querying the variable with the largest $\delta$-noisy influence.  By the results of the previous sections, we should be able to show that by growing $T^\circ$ out to
\[ \text{depth} = O\left(\frac{\log s}{\delta\eps^2}\right), \quad \text{and hence size} = s^{O(1/\delta\eps^2)}, \] 
it will be the case that all but an $\eps$-fraction of the paths $\pi$ of $T^\circ$ must satisfy $\Var((f_\pi)_\delta)\le \eps$, i.e.:  
\begin{equation} \Prx_{\bpi \in T^\circ}\big[\Var((f_{\bpi})_\delta) > \eps\big] \le \eps. \label{eq:low-variance} 
\end{equation}
On the other hand, by~\Cref{fact:stabilize}, noise sensitivity can only {\sl decrease} (in expectation) when variables are queried, and so 
\begin{equation} \Ex_{\bpi\in T^{\circ}}\big[\NS_\delta(f_{\bpi})\big] \le \NS_\delta(f) \le \kappa. \label{eq:low-NS}
\end{equation} 
Let $T$ be the completion of $T^\circ$ obtained by labeling the leaf at the end of each path $\pi$ with $\E[(f_\pi)_\delta]$.  Together~\Cref{eq:low-variance,eq:low-NS} should allow us to conclude that $\mathrm{error}_f(T) \le \poly(\eps) + \poly(\kappa)$. 



\begin{corollary}[Every small-depth DT has a variable of large noisy influence]
\label{cor:noisy-OSSS-truncated}
Let $f : \pmo^n \to \pmo$ be computable a size-$s$ decision tree.  Then there is an $i\in [n]$ such that 
\[ \Inf^{(1-2\delta)}_i(f^{\leq d}) \ge \frac1{(1-2\delta)^3}\cdot  \frac{\Var(f^{\leq d}_\delta)}{\log s} \ge \frac{\Var(f^{\leq d}_\delta)}{\log s}.\] 
\end{corollary} 

Consequently, as long as $\Var(f^{\leq d}_\delta) \ge \eps$, we are guaranteed the existence of a variable with $\delta$-noisy influence at least 
\[ \Inf_i^{(1-2\delta)}(f^{\leq d}) \ge \frac{\eps}{\log s}.\] 
\begin{proof}[Proof of~\Cref{cor:noisy-OSSS-truncated}]
Applying~\Cref{thm:OSSS} with $T$ being the size-$s$ DT that computes $f$, and $g$ being $f^{\leq d}_\delta$, we get that 
\begin{equation} \Cov(f,f^{\leq d}_\delta) \le \sum_{i=1}^n \delta_i(T) \cdot \Inf_i(f^{\leq d}_\delta) \le  \max_{i\in [n]}\Big\{ \Inf_i(f^{\leq d}_\delta)\Big\}\cdot \log s. \label{eq:apply-OSSS}
\end{equation} 
%
Next note that the LHS can be lower bounded by:
%
\begin{align*}  \Cov(f,f^{\leq d}_\delta) &= \sum_{S\ne \emptyset, |S|\leq d} (1-2\delta)^{|S|} \wh{f}(S)^2  \tag*{(Fourier expansion of $f_\delta$ (\ref{eq:smooth-fourier}) and formula for covariance (\ref{eq:covariance}))}\\
%
&\ge \frac1{1-2\delta}\cdot  \sum_{S\ne \emptyset, |S| \leq d} (1-2\delta)^{2|S|}\wh{f}(S)^2 \tag*{(since $(1-2\delta)^{2k} \le (1-2\delta)^{k+1}$ for all $k\ge 1$)}  \\
&= \frac{1}{1-2\delta} \cdot \Var(f^{\leq d}_\delta).  \tag*{(Formula for variance (\ref{eq:covariance}))}
\end{align*} 
On the other hand, we also have that 
\begin{align*}
 \Inf_i(f^{\leq d}_\delta) &= \sum_{S \ni i, |S| \leq d} (1-2\delta)^{2|S|} \wh{f}(S)^2  \tag*{(Formula for influence (\ref{eq:influence}))} \\
 &\le (1-2\delta)^2 \cdot \sum_{S \ni i, |S| \leq d} (1-2\delta)^{|S|-1} \wh{f}(S)^2 \tag*{(since $(1-2\delta)^{2k} \le (1-2\delta)^{k+1}$ for all $k\ge 1$)}  \\
 &= (1-2\delta)^2 \cdot \Inf^{(1-2\delta)}_i(f^{\leq d}).  \tag*{(Formula for $\delta$-noisy influence (\ref{eq:noisy-inf-fourier}))}
 \end{align*} 
 These two inequalities along with~\Cref{eq:apply-OSSS} give us 
 \[ \frac1{1-2\delta}\cdot \Var(f^{\leq d}_\delta) \le \max_{i\in [n]}\Big\{ \Inf_i^{(1-2\delta)}(f^{\leq d})\Big\} \cdot (1-2\delta)^2 \cdot \log s. \] 
 Rearranging completes the proof. 
\end{proof} 


==> intro.tex <==

%!TEX root = noisy.tex


\newcommand{\BuildStabilizingDT}{\textsc{BuildStabilizingDT}}
\newcommand{\StabilizingDT}{\textsc{StabilizingDT}}
\newcommand{\error}{\mathrm{error}}
\renewcommand{\hat}{\wh}
\renewcommand{\bn}{\pmo^n}
\renewcommand{\bits}{\pmo}

\title{Universal guarantees for decision tree induction\\
via a higher-order splitting criterion}

\date{\small{\today}}

\maketitle


\begin{abstract}
We propose a simple extension of {\sl top-down decision tree learning heuristics} such as~ID3, C4.5, and CART.  Our algorithm achieves provable guarantees for all target functions $f: \bn \to \bits$ with respect to the uniform distribution,  circumventing impossibility results showing that existing heuristics fare poorly even for simple target functions.   The crux of our extension is a new splitting criterion that takes into account the correlations between $f$ and {\sl small subsets} of its attributes. The splitting criteria of existing heuristics (e.g.~Gini impurity and information gain), in contrast, are based solely on the correlations between~$f$ and its {\sl individual} attributes.  

Our algorithm satisfies the following guarantee: for all target functions $f : \bn \to \bits$, sizes $s\in \N$, and error parameters $\eps$, it constructs a decision tree of size $s^{\tilde{O}((\log s)^2/\eps^2)}$ that achieves error $\le O(\opt_s) + \eps$, where $\opt_s$ denotes the error of the optimal size-$s$ decision tree.  A key technical notion that drives our analysis is the {\sl noise stability} of~$f$, a well-studied smoothness measure.


%We show that for a wide range of parameters, the runtime of our algorithm is optimal among all statistical query algorithms for learning decision trees.
 \end{abstract} 

%\thispagestyle{empty}
%
%\newpage 
%\setcounter{page}{1}

\section{Introduction} 

Decision trees have long been a workhorse of machine learning.  Their simple hierarchical structure makes them appealing in terms of interpretability and explanatory power.  They are fast to evaluate, with running time and query complexity both scaling linearly with the depth of the tree.  Decision trees remain ubiquitous in everyday machine learning applications, and they are at the heart of modern ensemble methods such as random forests~\cite{Bre01} and gradient boosted trees~\cite{CG16}, which achieve state-of-the-art performance in Kaggle and other data science competitions. 


\pparagraph{Top-down decision tree learning heuristics.} This focus of our work is on provable guarantees for widely employed and empirically successful {\sl top-down heuristics} for learning decision trees.  This includes well-known instantiations such as ID3~\cite{Qui86}, C4.5~\cite{Qui93}, and CART~\cite{Bre17}.   These heuristics proceed in a top-down fashion, greedily choosing a ``good'' attribute to query at the root of the tree, and building the left and right subtrees recursively.   In fact, all existing top-down heuristics are {\sl impurity-based}, and can be described in a common framework as follows.  Each heuristic is determined by a carefully chosen {\sl impurity function} $\mathscr{G}: [0,1] \to [0,1]$, which is restricted to be concave, symmetric around $\frac1{2}$, and to satisfy $\mathscr{G}(0) = \mathscr{G}(1) = 0$ and $\mathscr{G}(\frac1{2}) = 1$. Given examples $(\bx,f(\bx))$ labeled by  a target function $f:\bn \to \bits$, these heuristics query attribute $x_i$ at the root of the tree, where $x_i$ approximately maximizes the {\sl purity gain with respect to $\mathscr{G}$}: 
\[ \text{PurityGain\,}_{\mathscr{G},f}(x_i) \coloneqq \mathscr{G}(\dist_{\pm 1}(f)) - \Ex_{\bb\sim \bits}[ \mathscr{G}(\dist_{\pm 1}(f_{x_i=\bb}))], 
\] 
where $f_{x_i = b}$ denotes the subfunction of $f$ with its $i$-attribute set to $b$, and $\dist_{\pm 1}(f) \coloneqq \min\{\Pr[f(\bx) =1],\Pr[f(\bx) = -1]\}$. 
For example, ID3 and its successor C4.5 use the binary entropy function $\mathscr{G}(p) = \mathrm{H}(p)$ (the associated purity gain is commonly referred to as ``information gain''); CART uses the {\sl Gini criterion} $\mathscr{G}(p) = 4p(1-p)$; Kearns and Mansour, in one of the first papers to study impurity-based heuristics from the perspective of provable guarantees~\cite{KM99}, proposed and analyzed the impurity function $\mathscr{G}(p) = 2\sqrt{p(1-p)}$.  The high-level idea is that $\mathscr{G}(\dist_{\pm 1}(f))$ serves as a proxy for $\dist_{\pm 1}(f)$, the error incurred by approximating $f$ with the best constant-valued classifier.  (See the work of Dietterich, Kearns, and Mansour~\cite{DKM96} for a detailed discussion and experimental comparison of various impurity functions.) 

 \paragraph{An impossibility result for impurity-based heuristics.}  Given the popularity and empirical success of these top-down impurity-based heuristics, it is natural to seek broad and rigorous guarantees on their performance. Writing $\mathcal{A}_\mathscr{G}$ for the heuristic that uses $\mathscr{G}$ as its impurity function, ideally, one seeks a {\sl universal} guarantee for $\mathcal{A}_\mathscr{G}$: 
 
 \begin{quote}
 For {\sl all} target functions $f: \bn \to \bits$ and size parameters $s = s(n) \in \N$, the heuristic $\mathcal{A}_\mathscr{G}$ builds a decision tree of size not too much larger than $s$ that achieves error close to $\opt_s$, the error of the optimal size-$s$ decision tree for $f$. \hfill{$(\diamondsuit)$}
 \end{quote}


 Unfortunately, it has long been known (see e.g.~\cite{Kea96}) that such a universal guarantee is provably unachievable by {\sl any} impurity-based heuristic.  To see this, we consider the uniform distribution over examples and observe that for {\sl all} impurity functions~$\mathscr{G}$, the attribute $x_i$ that maximizes $\mathrm{PurityGain}_{\mathscr{G},f}(x_i)$ is the one with the highest correlation with $f$: 
\begin{equation}  \quad \mathrm{PurityGain}_{\mathscr{G},f}(x_i) \ge \mathrm{PurityGain}_{\mathscr{G},f}(x_j) \quad \text{iff}\quad \E[f(\bx)\bx_i]^2 \ge \E[f(\bx)\bx_j]^2. \label{eq:equivalence}
\end{equation}
(This is a straightforward consequence of the concavity of $\mathscr{G}$; see e.g.~Proposition 41 of~\cite{BLT20-ITCS}.\footnote{Proposition 41 of~\cite{BLT20-ITCS} is stated for monotone functions $f$, but its proof does not rely on the monotonicity of $f$.}) Now consider the target function $f(x) = x_i \oplus x_j$, the parity of two unknown attributes $i,j\in [n]$.  On one hand, this function $f$ is computed exactly by a decision tree with $4$ leaves (i.e.~$\opt_4=0$).  One the other hand, since $\E[f(\bx)\bx_k] = 0$ for all $k \in [n]$, {\sl any} impurity-based heuristic $\mathcal{A}_\mathscr{G}$---regardless of the choice of $\mathscr{G}$---may build a complete tree of size $\Omega(2^n)$ before achieving any non-trivial error.   

\paragraph{Prior work: provable guarantees for restricted classes of target functions.}  In light of such impossibility results, numerous prior works have focused on understanding the performance of impurity-based heuristics when run on {\sl restricted} classes of target functions.  Fiat and Pechyony~\cite{FP04} studied target functions that are halfspaces and read-once DNF formulas under the uniform distribution; recent work of Brutzkus, Daniely, and Malach~\cite{BDM19} studies read-once DNF formulas under product distributions, and provides theoretical and empirical results on the performance of a variant of ID3 introduced by Kearns and Mansour~\cite{KM99}.  In a different work~\cite{BDM19-smooth}, they show that ID3 learns $(\log n)$-juntas in the setting of smoothed analysis.   Recent works of Blanc, Lange, and Tan~\cite{BLT20-ITCS,BLT3} focus on provable guarantees for monotone target functions.  (We discuss other related work in~\Cref{sec:related}.) 


\subsection{Our contributions}   

We depart from the overall theme of prior works: instead of analyzing the performance of impurity-based heuristics when run on restricted classes of target functions, we propose a simple and efficient extension of these heuristics, and show that it achieves the sought-for universal guarantee~($\diamondsuit$).  In more detail, our main contributions are as follows: 

\begin{enumerate}[leftmargin=20pt]
\item {\sl A higher-order splitting criterion.} Recalling the equivalence (\ref{eq:equivalence}), the splitting criteria of impurity-based heuristics are based solely on the correlations between $f$ and its {\sl individual} attributes.  Our splitting criterion is a generalization that takes into account the correlations between $f$ and {\sl small subsets} of its attributes.  Instead of querying the attribute $x_i$ that maximizes $\E[f(\bx)\bx_i]^2$, our algorithm queries the attribute $x_i$ that maximizes: 
\[ \mathop{\sum_{S \ni i}}_{|S| \le d} (1-\delta)^{|S|} \textstyle \E\big[f(\bx)\prod_{i\in S}\bx_i\big]^2, \tag{$\star$}\] 
where $\delta \in (0,1)$ is an input parameter of the algorithm (and $d = \Theta(1/\delta)$).  This quantity aggregates the correlations between $f$ and subsets of attributes of size up to $d$ containing~$i$, where correlations with small subsets contribute more than those with large ones due to the attenuating factor of $(1-\delta)^{|S|}$.

\item {\sl An algorithm with universal guarantees.}  We design a simple top-down decision tree learning algorithm based on our new splitting criterion ($\star$), and show that it achieves provable guarantees for all target functions $f : \bn \to \bits$, i.e.~a universal guarantee of the form ($\diamondsuit$).  This circumvents the impossibility results for impurity-based heuristics discussed above.  

%Furthermore, we show that our algorithm achieves stronger guarantees for monotone target functions, again circumventing impossibility results that~\cite{BLT3} had shown for impurity-based heuristics when run on such target functions. 

\item {\sl Decision tree induction as a noise stabilization procedure.}  Noise stability is a well-studied smoothness measure of a function $f$ (see~e.g.~Chapter \S2.4 of~\cite{ODbook}).  Roughly speaking, it measures how often the output of $f$ stays the same when a small amount of noise is applied to the input. Strong connections between noise stability and learnability have long been known~\cite{KOS04,KKMS08}, and our work further highlights its utility in the specific context of top-down decision tree learning algorithms.  

Indeed, our algorithm can be viewed as a ``noise stabilization'' procedure.  Recalling that each query in the decision tree splits the dataset into two halves, the crux of our analysis is a proof that the average noise stability of both halves is significantly higher than that of the original dataset.  Therefore, as our algorithm grows the tree, it can be viewed as refining the corresponding partition of the dataset so that the parts become more and more noise stable.   Intuitively, since constant functions are the most noise stable, this is how we show that our algorithm makes good progress towards reducing classification error.

Our algorithm and its analysis are inspired by ``noisy-influence regularity lemmas" from computational complexity theory~\cite{OSTW10,Jon16}. 
\end{enumerate}

\subsection{Formal statements of our algorithm and main result} 


\paragraph{Feature space and distributional assumptions.}  We will work in the setting of binary attributes and binary classification, i.e.~we focus on the task of learning a target function $f : \bn \to \bits$.  We will assume that our learning algorithm receives labeled examples $(\bx,f(\bx))$ where $\bx \sim \bn$ is uniform random, and the error of a hypothesis $T : \bn \to \bits$ is defined to be $\error_f(T) \coloneqq \Pr[f(\bx) \ne T(\bx)]$ where $\bx\sim \bn$ is uniform random.  We write $\opt_s(f)$ to denote $\min\{ \error_f(T) \colon \text{$T$ is a size-$s$ decision tree} \}$; when $f$ is clear from context we simply write $\opt_s$. 

\paragraph{Notation and terminology.}  For any decision tree $T$, we say the size of $T$ is the number of leaves in $T$. We refer to a decision tree with unlabeled leaves as a {\sl partial tree}, and write $T^\circ$ to denote such trees.  We call any decision tree $T$ obtained from $T^\circ$ by a labeling of its leaves a {\sl completion} of $T^\circ$.  Given a partial tree $T^\circ$ and a target function $f : \bn\to \bits$, there is a canonical completion of $T^\circ$ that minimizes classification error $\error_f(T)$: label every leaf $\ell$ of $T^\circ$ with $\sign(\E[f_\ell])$, where $f_\ell$ denotes the subfunction of $f$ obtained by restricting its attributes according to the path that leads to $\ell$.  We write $T^\circ_f$ to denote this canonical completion, and call it the {\sl $f$-completion of~$T^\circ$}.  For a leaf $\ell$ of a partial tree $T^\circ$, we write $|\ell|$ to denote its depth within~$T^\circ$, the number of attributes queried along the path that leads to $\ell$.  We will switch freely between a decision tree $T$ and the function $T : \bn \to \bits$ that it represents. 

We use {\bf boldface} to denote random variables (e.g.~`$\bx$'), and unless otherwise stated, all probabilities and expectations are with respect to the uniform distribution. 

\paragraph{Fourier analysis of boolean functions.}  We will draw on notions and techniques from the Fourier analysis of boolean functions; for an in-depth treatment of this topic, see~\cite{ODbook}.  Every function $f : \bn \to \R$ can be uniquely expressed as a multilinear polynomial via its {\sl Fourier expansion}: 
\begin{equation} f(x) = \sum_{S\sse [n]} \hat{f}(S) \prod_{i\in S}x_i, \quad \textstyle \text{where $\hat{f}(S) = \E\big[f(\bx)\prod_{i\in S}\bx_i\big]$}. \label{eq:fourier-expansion}
\end{equation} 
\begin{definition}[$\delta$-noisy influence]
\label{def:stable-influence} 
For a function $f : \bn \to \R$ and a coordinate $i\in [n]$, the {\sl $\delta$-noisy influence of $i$ on $f$} is the quantity 
\begin{equation*}
 \Inf_i^{(\delta)}(f) \coloneqq \sum_{S \ni i} (1-\delta)^{|S|}\hat{f}(S)^2. 
 \end{equation*}
The {\sl $\delta$-noisy $d$-wise influence of $i$ on $f$} is the quantity
\[ \Inf_i^{(\delta,d)}(f) \coloneqq \mathop{\sum_{S\ni i}}_{|S|\le d} (1-\delta)^{|S|}\hat{f}(S)^2. \] 
\end{definition} 

We are now ready to state our algorithm and main result: 



\begin{figure}[H]
  \captionsetup{width=.9\linewidth}
\begin{tcolorbox}[colback = white,arc=1mm, boxrule=0.25mm]
\vspace{3pt} 

$\BuildStabilizingDT_f(t,\delta,\eps)$:  \vspace{6pt} 

\ \ Initialize $T^\circ$ to be the empty tree. \vspace{4pt} 

\ \ while ($\size(T^\circ) < t$) \{  \\

\vspace{-15pt}
\begin{enumerate} 
\item {\sl Score:}  For every leaf $\ell$ in $T^\circ$, let $x_i$ denote the attribute with the largest $\delta$-noisy $d$-wise influence on the subfunction $f_\ell$ where $d \coloneqq \log(1/\eps)/\delta$: 
\[ \Inf^{(\delta,d)}_i(f_\ell) \ge \Inf^{(\delta,d)}_j(f_\ell) \quad \text{for all $j\in [n]$.} \] 
Assign $\ell$ the score: 
\[ \score(\ell) \coloneqq \Prx_{\bx\sim\pmo^n}[\,\text{$\bx$ reaches $\ell$}\,] \cdot \Inf_i^{(\delta,d)}(f_\ell) = 2^{-|\ell|} \cdot \Inf^{(\delta,d)}(f_\ell). \] 
\item {\sl Split:} Let $\ell^\star$ be the leaf with the highest score, and $x_{i}^\star$ be the associated high noisy-influence attribute.  Grow $T^\circ$ by splitting $\ell$ with a query to $x_{i^\star}$. 

\end{enumerate} 
\ \ \}  \vspace{4pt} 

\ \ Output the $f$-completion of $T^\circ$.
\vspace{3pt}
\end{tcolorbox}
\caption{$\BuildStabilizingDT$ has access to uniform random examples $(\bx,f(\bx))$ of a target function $f : \bn\to\bits$, and outputs a size-$T$ decision tree hypothesis.}
\label{fig:TopDown}
\end{figure}


%Our most general algorithmic guarantee bounds the performance of $\BuildStabilizingDT_f$ in terms of the {\sl noise sensitivity} of $f$, a well-studied smoothness measure of $f$:
%
%\begin{definition}[Noise sensitivity] 
%For $f : \bn\to\bits$ and $\delta \in (0,1)$, the {\sl noise sensitivity of $f$ at noise rate $\delta$} is the quantity $\NS_\delta(f) \coloneqq \Pr[f(\bx)\ne f(\tilde{\bx})]$, where $\bx\sim \bn$ is uniform random, and $\tilde{\bx}$ is obtained from $\bx$ by rerandomizing each of its coordinates independently with probability $\delta$.\footnote{The notion of ``noise stability" we referred to in our introduction can be defined to be $1-\NS_\delta(f)$, though we will work exclusively with noise sensitivity throughout this paper.} 
%\end{definition}  
%
%\begin{theorem}[Most general algorithmic guarantee] 
%\label{thm:main} 
%Let $f : \pmo^n \to \bits$ be such that $\NS_\delta(f) \le \kappa$.  For all $s \in \N$ and $\eps,\delta \in (0,\frac1{2})$, by choosing $t = s^{O(\kappa/\eps\delta)}$,
%$\BuildStabilizingDT_f(t,\delta,\eps)$ runs in time $(n+s)^{O(1/\delta\eps)}$ and returns a tree $T$ of size $t$ satisfying $\error_f(T) \le O(\opt_s) + \kappa +\eps$.  
%\end{theorem} 
%
%
% We derive three corollaries of~\Cref{thm:main}: 

\begin{theorem}[Main result]
\label{thm:universal} 
Let $f : \pmo^n \to \bits$ be any target function.  For all $s\in \N$, $\eps \in (0,\frac1{2})$, and $\delta = \eps / (\log s)$, $\BuildStabilizingDT_f$ runs in time $(ns)^{\tilde{O}((\log s)^2/\eps^2)}$ and returns a tree $T$ of size $s^{\tilde{O}((\log s)^2/\eps^2)}$ satisfying $\error_f(T) \le O(\opt_s) +\eps$.  
\end{theorem} 

\Cref{thm:universal} should be contrasted with the impossibility result discussed in the introduction, which shows that there are very simple target functions for which $\opt_4 = 0$, and yet any impurity-based heuristic may build a complete tree of size $\Omega(2^n)$ (in time $\Omega(2^n)$) before achieving any non-trivial error $(< \frac1{2})$.  Hence,~\Cref{thm:universal} shows the increased power of our new splitting criterion. 


%\begin{corollary}[Monotone target functions] 
%\label{cor:monotone} 
%Let $f: \bn\to\bits$ be a monotone target function.  For all $s\in \N$ and $\eps \in (0,\frac1{2})$, $\BuildStabilizingDT_f$ can be instantiated so that it runs in time $(n+s)^{O((\log s)/\eps^2)}$ and returns a tree of size $s^{O((\sqrt{\log s})/\eps^2)}$ satisfying $\error_f(T) \le O(\opt_s) + \eps$.
%\end{corollary} 
%
%\Cref{cor:monotone} should be compared to the main result of~\cite{BLT3}, who shows that for monotone target functions $f$, impurity-based heuristics run in time $\poly(n, s^{O((\log s)/\eps^2)})$ and return a tree of size $s^{O((\log s)/\eps^2)}$ that achieves error $\le \opt_s + \eps$.~\cite{BLT3} also provide a near-matching lower bound, showing that there are monotone $f$'s and values of $s$ for which $\opt_s \le 0.01$, and yet any impurity-based heuristic has to grow a tree of size $s^{\tilde{\Omega}(\log s)}$ before achieving error $\le 0.49$. 
%
%Our final corollary concerns {\sl asymptotically noise stable} target function classes~\cite{BKS99}: these are function classes $\{ f_n : \bn \to\bits\}_{n\in \N}$ for which $\NS_\delta(f_n) \le \Phi(\delta)$ where $\Phi$ is a function that is independent of $n$, and goes to $0$ as $\delta \to 0$.  Function classes that have been shown to be asymptotically noise stable include halfspaces~\cite{Per04}, constant-degree threshold functions~\cite{DRST10}, and intersections of constantly-many halfspaces~\cite{KOS04,Kan14-polytopes}. 
%
%\begin{corollary}[Asymptotically noise stable target functions] 
%\label{cor:noise-stable-targets} 
%Let $f: \bn\to\bits$ belong to an asymptotically noise stable target function class.  For all $s \in \N$ and $\eps \in (0,\frac1{2})$,  $\BuildStabilizingDT_f$ can be instantiated so that it runs in time $(n+s)^{O_\eps(1)}$ and returns a tree $T$ of size $s^{O_\eps(1)}$ satisfying $\error_f(T) \le O(\opt_s) + \eps$. 
%\end{corollary} 
%
%Hence, for constant values of $\eps$, the running time is $\poly(n,s)$ and decision tree size is $\poly(s)$ (where the constants in the exponents depend on the $\Phi$'s of the corresponding function class). 


\begin{remark}[Estimating noisy influence from random labeled examples] 
For all values of $d,i,$ and $\delta$, the quantity $\Inf_i^{(\delta,d)}(f)$ can be estimated to high accuracy from uniform random examples $(\bx,f(\bx))$ in time $n^{O(d)}$ via the identity (\ref{eq:fourier-expansion}).  More generally, $\Inf_i^{(\delta,d)}(f_\ell)$ can be estimated to high accuracy in time $\poly(2^\ell,n^d)$.  In our analysis we will assume that these quantities can be computed {\sl exactly} in time $\poly(2^{\ell},n^d)$, noting that the approximation errors can be easily incorporated into our analysis via standard methods. 
\end{remark} 



%\pparagraph{Matching SQ lower bounds.}  Our algorithm falls within the broad and well-studied statistical query (SQ) framework~\cite{Kea98}.  We complement~\Cref{thm:main} with a matching SQ lower bound, showing that for a wide range of parameters, the runtime of our algorithm is optimal among all SQ algorithms (even in the realizable setting, and for the easier task of weak learning). 

% \subsection{Other related work}
% \label{sec:related} 
% Kearns and Mansour~\cite{KM99} (see also~\cite{Kea96}) analyzed top-down impurity-based heuristics from the perspective of {\sl boosting}, where the attributes queried in the tree are viewed as weak hypotheses.  As is standard in results on boosting, their results are conditional in nature: they assume the existence of weak hypotheses for all filtered-and-rebalanced versions of the original distribution.  (In contrast, we carry out the entirety of our analysis over the uniform distribution.) 

% Recent work of Blanc et al.~\cite{BLT20-ITCS} gives a top-down algorithm for learning decision trees that achieves provable guarantees for all target functions $f$.  However, their algorithm makes crucial use of {\sl membership queries}, which significantly limits its practical applicability and relevance.  Furthermore, their guarantees only hold in the realizable setting,  requiring that $f$ is itself a size-$s$ decision tree (i.e.~$\opt_s = 0$).  

% There has been extensive work in the learning theory literature on learning target functions that are decision trees~\cite{EH89,Blu92,KM93,OS07,GKK08,HKY18,CM19}.  However, none of these algorithms proceed in a top-down manner like the practical heuristics that are the focus of this work; indeed, with the exception~\cite{EH89}, these algorithms do not return a decision tree as their hypothesis. (\cite{EH89}'s algorithm constructs its decision tree hypothesis in a {\sl bottom-up} manner.)







==> lowerbound.tex <==
\section{Lower Bound}

We prove lower bounds showing that our algorithm is competitive with any learning algorithm in the statistical query framework introduced by Kearns \cite{Kea98}.
\begin{definition}[Statistical Query]
    A statistical query of a function $f: \bn \to \pm 1$ is defined by function $\phi: \bn \times \{\pm 1\} \to \{\pm 1\}$ and tolerance $\tau \in [0,1]$. The query returns any value $v$ satisfying
    \begin{align*}
        \left|\Ex_{\bx \in \bn}[\phi(\bx, f(\bx))] - v\right| \leq \tau
    \end{align*}
\end{definition}


Most known learning algorithms with provable guarantees that take as input random examples labeled from $f$ and output an approximation to $f$ can be reformulated as instead using statistical queries of $f$.\footnote{One prominent learning algorithm that does \textit{not} use statistical queries is that of learning parities using Gaussian Elimination} Our algorithm is no exception. The only information about $f$ that our algorithm needs is estimates of the noisy influence of each variable on subfunctions of $f$. By \Cref{eq:fourier-expansion}, those estimates can be computed using sufficiently high accuracy of statistical queries of $f$ where $\phi$ is of the form:
\begin{align*}
    \phi(x, y) = \Ind[x \in \ell] \cdot f(x) \prod_{i \in S} x_i
\end{align*}
for appropriately chosen $\ell$, corresponding to the subfunction who's noisy influences we are estimating, and $S$, corresponding to the particular Fourier coefficient we are estimating. 

Any algorithm that uses $q$ efficient\footnote{By ``efficient," we mean that $\phi$ uses time $\poly(q, \frac{1}{\tau})$. Generally, $\phi$ is very simple and quick to compute.} statistical queries of accuracy $\tau$ corresponds to a learning algorithm that receives $\poly(q, \frac{1}{\tau})$ random labeled samples of $f$ and runs in time $\Theta(\poly(q, \frac{1}{\tau}))$. That corresponding learning algorithm directly estimates the statistical queries using the labeled samples. The above observation leads to a popular lower bound technique within learning theory. By showing that $\poly(t)$ statistical queries of tolerance $\poly(\frac{1}{t})$ are not enough to learn a function class, one effectively proves that any learning algorithm based purely on statistical queries can not learn that function class in time $O(t)$.


\begin{fact}[Direct consequence of Theorem 12 in \cite{BFJKMR94}]
    \label{fact:parities are hard in SQ}
    Let $\mathcal{F}$ be a collection of target functions, each $\bn \to \{\pm 1\}^n$ that, for any $k < n$, contains all parities of $k$ variables. Let $\mathcal{A}$ be any statistical query learning algorithm that, for
    \begin{align*}
        t = \poly\left( \binom{n}{k} \right ),
    \end{align*} 
     makes at most $t$ statistical queries of tolerance at least $\frac{1}{t}$. There is at least one $f \in \mathcal{F}$ on which $\mathcal{A}$ returns a hypothesis with error at least $\frac{1}{2} - \frac{1}{t}$.
\end{fact}

We leverage \Cref{fact:parities are hard in SQ} to show that, for a range of parameters, our upper bound in \Cref{thm:main} is optimal among all statistical query algorithms. In addition to ruling out the possibility of any algorithm with the statistical query framework achieving a better runtime, since our algorithm is a statistical query algorithm, it proves our upper bound analysis tight.
\begin{lemma}
    \label{lemma:lower bound}
    Fix a constant $\kappa \in (0, 0.49)$. For any $n$ and $k \leq O(\log(n))$, let $\delta = \frac{\kappa}{k}$, and $s = 2^k$. If $\mathcal{A}$ is any statistical query algorithm, that, for any size-$s$ decision tree $f$ with $\NS_\delta(f) \leq \kappa$, outputs a hypothesis with error less than $0.49$, then $\mathcal{A}$ must make either $t$ queries or make a query with tolerance $\frac{1}{t}$ for
    \begin{align}
        \label{eq: t from lower bound}
        t = (n + s)^{\Omega_\kappa(\frac{1}{\delta})}.
    \end{align}
\end{lemma}
For the parameters above, \Cref{thm:main} needs only $(n + s)^{O(\frac{1}{\delta})}$ statistical queries of tolerance $(n + s)^{-\Omega(\frac{1}{\delta})}$ to output a hypothesis with error only $0.01$ (better than the $0.49$ lower bound in \Cref{lemma:lower bound}). Hence, this lower bound matches our upper bound up to constants in the exponent.
\begin{proof}
    Let $\mathcal{F}$ be the set of all size-$s$ decision trees $f$ with $\NS_\delta(f) \leq \kappa$. We first show that $\mathcal{F}$ contains all parities of $k$ variables. 
    
    Any parity of $k$ variables is a size $s = 2^k$ decision tree. Furthermore, let $f$ be any parity over $k$ variables and $S$ be those $k$ variables. For $\bx \in \bn$ uniform random and $\tilde{\bx}$ is obtained from $\bx$ by rerandomizing each of its coordinates independently with probability $\delta$,
    \begin{align*}
        \NS_\delta(f) &= \Pr[f(\bx)\ne f(\tilde{\bx})] \\
        &\leq \Pr[\text{At least one coordinate in $S$ is rerandomized}]\\
        &\leq \delta \cdot k \\
        & \leq \kappa.
    \end{align*}
    Hence, $\mathcal{F}$ contains all parities of $k$ variables. By \Cref{fact:parities are hard in SQ}, any statistical query algorithm that, for $t = \poly(\binom{n}{k})$, makes only $t$ queries of tolerance $\frac{1}{t}$ can not achieve accuracy $0.49$ (for sufficiently large $t$).
    
    We manipulate this $t$ to show it can be written in the same form as \Cref{eq: t from lower bound}.
    \begin{align*}
        t &= \poly(\binom{n}{k}) \\
        &= \left(\frac{n-k}{k}\right)^{\Omega(k)} \\
        &= \left(\sqrt{n}\right)^{\Omega(k)} \tag*{$k = O(\log(n)) \implies \frac{n - k}{k} = \Omega(\sqrt{n})$}\\
        &= \left(n \right)^{\Omega(k)} \tag*{change constant in $\Omega(\cdot)$}\\
        &= \left(n + s\right)^{\Omega(k)} \tag*{$s = \poly(n)$ and change constant in $\Omega(\cdot)$}\\
        &= \left(n + s\right)^{\Omega_\kappa(\frac{1}{\delta})} \tag*{$k = \frac{\kappa}{\delta}$}.
    \end{align*}
\end{proof}

==> preliminaries_shortened.tex <==


%!TEX root = noisy.tex



\paragraph{Other useful definitions and identites from the Fourier analysis of boolean functions.} 
%Every function $f : \pmo^n \to \R$ can be expressed as a polynomial via its {\sl Fourier expansion}: 
%\[ f(x) = \sum_{S\sse [n]}\wh{f}(S) \prod_{i\in S}x_i. 
%\] 
%The {\sl $i$-th discrete derivative} of $f : \pmo^n \to \R$ is the function
%\[ (D_i f)(x) = \frac{f(x^{i=1}) - f(x^{i=-1})}{2}.\] 
%The {\sl influence of $i$ on $f$} is the quantity 
%\begin{equation} \Inf_i(f) = \E\big[(D_i f)(\bx)^2\big] = \sum_{S \ni i} \wh{f}(S)^2. \label{eq:influence}
%\end{equation} 
% In the case of boolean-valued functions $f : \pmo^n \to \pmo$, we have the combinatorial interpretation $\Inf_i(f) = \Pr[f(\bx) \ne f(\bx^{\oplus i})]$.   
 
 
 For $f : \bn\to\R$, we have Parseval's identity, 
 \begin{equation} \sum_{S\sse [n]}\hat{f}(S)^2 = \E[f(\bx)^2].\label{eq:Parseval} 
 \end{equation} 
 In particular, for $f : \bn\to\bits$ we have that $\sum_{S\sse [n]}\hat{f}(S)^2 = 1$.  
 The {\sl variance of $f$} is given by the formula 
\begin{equation} \Var(f) \coloneqq \E[f(\bx)^2] - \E[f(\bx)]^2 = \sum_{S \ne \emptyset} \wh{f}(S)^2. \label{eq:variance}
\end{equation} 
%\gray{More generally, the covariance of $f,g : \pmo^n \to \R$ is given by the formula 
%\begin{equation} \Cov(f,g) = \sum_{S \ne \emptyset} \wh{f}(S)\wh{g}(S) = \lfrac{1}{2}\big(\E[(f(x)-g(y))^2]-\E[(f(x)-g(x))^2]
%\big). \label{eq:covariance}
%\end{equation} }
For $x\in\bn$, we write $\tilde{\bx} \sim_\delta x$ to denote a {\sl $\delta$-noisy copy of $x$}, where $\tilde{\bx}$ is obtained by rerandomizing each coordinate of $x$ independently with probability $\delta$.  (Equivalently, $\tilde{\bx}$ is obtained by flipping each coordinate of $x$ independently with probability $\lfrac{\delta}{2}$.)
% $(x,\tilde{\bx})$ are $(1-\delta)$-correlated, meaning $\E[x_i\tilde{\bx}_i] = 1-\delta$ for all $i\in [n]$.
 For $f : \pmo^n \to \bits$ and $\delta \in (0,1)$, we define the {\sl $\delta$-smoothed version of $f$} to be $f_\delta : \bn \to [-1,1]$, 
\begin{equation} f_{\delta}(x) \coloneqq \Ex_{\tilde{\bx}\sim_{\delta}x}[f(\tilde{\bx})] = \sum_{S\sse [n]} (1-\delta)^{|S|} \wh{f}(S)\prod_{i\in S}x_i. \label{eq:smooth-fourier}
\end{equation} 
For $g : \bn\to\R$, we write $g^{\le d} : \bn\to \R$ to denote the degree-$d$ polynomial that one obtains by truncating $g$'s Fourier expansion to degree $d$: $ g^{\leq d}(x) = \mathop{\sum_{S\sse [n]}}_{|S|\le d} \hat{g}(S) \prod_{i\in S} x_i.$
%
The {\sl $i$-th discrete derivative} of $g : \pmo^n \to \R$ is the function
\[ (D_i g)(x) \coloneqq \frac{g(x^{i=1}) - g(x^{i=-1})}{2} = \sum_{S\ni i}\hat{g}(S) \prod_{j \in S\setminus \{ i\}} x_j,\]
where $x^{i=b}$ denotes $x$ with its $i$-th coordinate set to $b$.  
\begin{definition}[Defining influence in terms of derivatives] 
\label{def:influence} 
For $g : \bn \to \R$ and $i\in [n]$, the {\sl influence of $i$ on $g$} is the quantity 
\[ \Inf_i(g) \coloneqq \E[(D_i g)(\bx)^2] = \sum_{S\ni i} \hat{g}(S)^2.\] 
We define the {\sl $\delta$-noisy influence of $i$ on $g$} to be the quantity 
\[ \Inf_i^{(\delta)}(g) \coloneqq (1-\delta) \mathop{\Ex_{\bx\sim\bn}}_{\tilde{\bx}\sim_\delta\bx}[(D_i g)(\bx)(D_ig)(\tilde{\bx})] = \sum_{S\ni i} (1-\delta)^{|S|} \hat{g}(S)^2,\] 
and the {\sl $\delta$-noisy $d$-wise influence of $i$ on $g$} to be $\Inf_i^{(\delta,d)}(g) \coloneqq \Inf_i^{(\delta)}(g^{\le d})$.
\end{definition} 



%
%%%%
%%%\gray{
%%%$$\E[(D_if)(\bx)(D_if)(\tilde{\bx})] = \sum_{S \ni i}(1-\delta)^{|S|-1}\hat{f}(S)^2 = \frac{1}{1-\delta}\Inf_i^{(\delta)}(f)$$
%%%\begin{enumerate}
%%%\item $x^{\oplus i}$
%%%\item $\opt$-close
%%%\end{enumerate} 
%%%}
\section{Our algorithm as a noise stabilization procedure} 

As alluded to in the introduction, our algorithm $\BuildStabilizingDT$ can be viewed as a  ``noise stabilization'' procedure.  Towards formalizing this, we begin by recalling the definition of noise sensitivity: 
\begin{definition}[Noise sensitivity of $f$] 
For $f : \bn\to\bits$ and $\delta \in (0,1)$, the {\sl noise sensitivity of $f$ at noise rate $\delta$} is the quantity $\NS_\delta(f) \coloneqq \Pr[f(\bx)\ne f(\tilde{\bx})]$, where $\bx\sim \bn$ is uniform random, and $\tilde{\bx}$ is obtained from $\bx$ by rerandomizing each of its coordinates independently with probability~$\delta$.\footnote{The notion of ``noise stability'' we referred to in our introduction is defined to be $1-2\,\NS_\delta(f)$, though we will work exclusively with noise sensitivity throughout this paper.} 
\end{definition}  

Noise sensitivity has been extensively studied (see e.g.~O'Donnell's Ph.D.~thesis~\cite{ODThesis03}); we will only need very basic properties of this notion, all of which is covered in Chapter \S2.4 of the book~\cite{ODbook}. 

We now introduce the potential function that will facilitate our analysis of $\BuildStabilizingDT$: 

\begin{definition}[Noise sensitivity of $f$ with respect to $T^\circ$] 
\label{def:NS-wrt-T} 
Let $f :\bn\to\bits$ be a function and $T^\circ$ be a partial decision tree.  The {\sl noise sensitivity of $f$ with respect to the partition induced by $T^\circ$} is the quantity 
\[ \NS_\delta(f,T^\circ) \coloneqq \sum_{\text{leaves $\ell \in T^\circ$}} \Pr[\,\text{$\bx$ reaches $\ell$}\,] \cdot \NS_\delta(f_\ell)  =  \sum_{\text{leaves $\ell \in T^\circ$}} 2^{-|\ell|} \cdot \NS_\delta(f_\ell).\] 
\end{definition} 


We observe that $\NS_\delta(f,T^\circ)$ where $T^\circ$ is the empty tree is simply $\NS_\delta(f)$, the noise sensitivity of $f$ at noise rate $\delta$.  The following fact quantifies the decrease in $\NS_\delta(f,T^\circ)$ when we split a leaf of $T^\circ$: 

\begin{fact}[Stability gain associated with a split] 
\label{fact:split-stabilize}
Let $f : \bn\to\bits$ be a function and $T^\circ$ be a partial decision tree.  Fix a leaf $\ell^\star$ of $T^\circ$ and a coordinate $i\in [n]$, and let $T^\circ_{\ell^\star \to x_i}$ denote the extension of $T^\circ$ obtained by splitting $\ell$ with a query to $x_i$.  We define 
\[ \mathrm{StabilityGain}_f(T^\circ,\ell^\star,i) \coloneqq \NS_{\delta}(f,T^\circ) - \NS_{\delta}(f,T^\circ_{\ell^\star\to x_i}). \] 
  Then 
\[ \mathrm{StabilityGain}_f(T^\circ,\ell^\star,i) =  \lfrac{\delta}{2(1-\delta)}\cdot \Inf_i^{(\delta)}(f_{\ell^\star}).\]
\end{fact}
We defer proof of~\Cref{fact:split-stabilize} to~\Cref{sec:Jones}. 

%%%\bigskip
%%%
%%%\bigskip
%%%
%%%\bigskip 
%%%
%%%From Fact \ref{fact:stabilize} , we know that
%%% \[\NS_{\delta}(f) = \lfrac{1}{2}\big(\NS_{\delta}(f_{x_i=-1}) + \NS_{\delta}(f_{x_i=1})\big) + \frac{\delta}{2(1-\delta)}\cdot \Inf^{(\delta)}_i(f).\] 
%%%%
%%%Using this we get that
%%%%
%%%\begin{align*}
%%%\NS_{\delta}(T',f) &= \sum_{\text{leaf } l \in T'}\frac{1}{2^{|l|}}\NS_{\delta}(f_l)\\
%%%&= \sum_{\text{leaf } l \in T}\frac{1}{2^{|l|}}\NS_{\delta}(f_{l}) + \frac{1}{2^{|l'|+1}}\NS_{\delta}(f_{l',x_{i}=0}) + \frac{1}{2^{|l'|+1}}\NS_{\delta}(f_{l', x_{i}=1}) -\frac{1}{2^{|l'|}}\NS_{\delta}(f_{l'})  \\
%%%&= \NS_{\delta}(T,f) - \frac{\delta}{2^{|l'|+1}(1-\delta)}\Inf_i^{(\delta)}(f_{l'})
%%%\end{align*}
%%%
%
%


%
%
%
%
%
%\bigskip
%
%\bigskip 
%
%\bigskip
%
%
%\begin{fact}[Corollary of Lemma 5 of \cite{Jon16}] 
%\label{fact:stabilize} 
% \[\NS_{\delta}(f) = \lfrac{1}{2}\big(\NS_{\delta}(f_{x_i=-1}) + \NS_{\delta}(f_{x_i=1})\big) + \frac{\delta}{2(1-\delta)}\cdot \Inf^{(\delta)}_i(f).\] 
%\end{fact} 
%%
%\begin{proof}
%\begin{align*}
%    \NS_{\delta}(f) &= \Pr[f(\bx) \neq f(\tilde{\bx})] = 1-\frac{1}{2}\E[f(\bx)f(\tilde{\bx})]\\
%    &= 1 - \frac{1}{2}\big(\frac{1}{2}\big(1-\frac{\delta}{2}\big)f({\bx}^{x_i=1})f(\tilde{\bx}^{x_i=1})+\frac{1}{2}\big(1-\frac{\delta}{2}\big)f({\bx}^{x_i=-1})f(\tilde{\bx}^{x_i=-1})\\
%    &+\frac{1}{2}\frac{\delta}{2}f({\bx}^{x_i=1})f(\tilde{\bx}^{x_i=-1})+\frac{1}{2}\frac{\delta}{2}f({\bx}^{x_i=-1})f(\tilde{\bx}^{x_i=1})\big)\\
%    &= 1 - \frac{1}{4}(f({\bx}^{x_i=1})f(\tilde{\bx}^{x_i=1})+f({\bx}^{x_i=-1})f(\tilde{\bx}^{x_i=-1}))\\
%    &+ \frac{\delta}{8}\big(f({\bx}^{x_i=1})f(\tilde{\bx}^{x_i=1})+f({\bx}^{x_i=-1})f(\tilde{\bx}^{x_i=-1}) -f({\bx}^{x_i=1})f(\tilde{\bx}^{x_i=-1})-f({\bx}^{x_i=-1})f(\tilde{\bx}^{x_i=1})\big)\\
%    %
%    &= \frac{1}{2}(\NS_{\delta}(f_{x_i=1})+\NS_{\delta}(f_{x_i=-1}))+ \frac{\delta}{2}\E[(D_if)(\bx)(D_if)(\tilde{\bx})]\\
%    &= \frac{1}{2}(\NS_{\delta}(f_{x_i=1})+\NS_{\delta}(f_{x_i=-1}))+ \frac{\delta}{2(1-\delta)}\Inf_i^{(\delta)}(f)\qedhere
%\end{align*}
%\end{proof}
%In words,~\Cref{fact:stabilize} says that the $\delta$-noise sensitivity of $f$ goes {\sl down} by an additive $
%\frac{\delta}{2(1-\delta)}\cdot \Inf_i^{(\delta)}(f)$ (in expectation) when $x_i$ is queried. %




==> proof_outline.tex <==
\section{Upper bound on size of {\sc BuildStabilizingDT} output}
\subsection{Potential function}

Our potential function of a function $f$ with respect to a partially grown tree $T$ would be denoted as $\Stability_{\delta}(T,f)$ where

$$\NS_{\delta}(T,f) = \sum_{\text{leaf } l \in T}\frac{1}{2^{|l|}}\NS_{\delta}(f_l)$$

\begin{fact}
\label{fact:stabilize-2}
Let $T$ be a partially grown decision tree and $T'$ be the extension of it by splitting the leaf $l'$ with the variable $i$, then
$$\NS_{\delta}(T',f) = \NS_{\delta}(T,f) - \frac{\delta}{2^{|l'|+1}(1-\delta)}\Inf_i^{(\delta)}(f_{l'})$$
\end{fact}

\begin{proof}
From Fact \ref{fact:stabilize} , we know that
 \[\NS_{\delta}(f) = \underbrace{\lfrac{1}{2}\big(\NS_{\delta}(f_{x_i=-1}) + \NS_{\delta}(f_{x_i=1})\big)}_{\text{Average noise sensitivity of restrictions}} + \frac{\delta}{2(1-\delta)}\cdot \Inf^{(\delta)}_i(f).\] 
%
Using this we get that
%
\begin{align*}
\NS_{\delta}(T',f) &= \sum_{\text{leaf } l \in T'}\frac{1}{2^{|l|}}\NS_{\delta}(f_l)\\
&= \sum_{\text{leaf } l \in T}\frac{1}{2^{|l|}}\NS_{\delta}(f_{l}) + \frac{1}{2^{|l'|+1}}\NS_{\delta}(f_{l',x_{i}=0}) + \frac{1}{2^{|l'|+1}}\NS_{\delta}(f_{l', x_{i}=1}) -\frac{1}{2^{|l'|}}\NS_{\delta}(f_{l'})  \\
&= \NS_{\delta}(T,f) - \frac{\delta}{2^{|l'|+1}(1-\delta)}\Inf_i^{(\delta)}(f_{l'})
\end{align*}
\end{proof}
%
\subsection{Maximum $\delta$-noisy influence variable}
%
%
\begin{corollary}[Every small-depth DT has a variable of large noisy influence]
\label{cor:noisy-OSSS-truncated-agnostic}
Let $f : \pmo^n \to \pmo$ be $OPT$ close to a size-$s$ decision tree $h$.  Then there is an $i\in [n]$ such that 
\[ \Inf^{(\delta, d)}_i(f) \ge \frac{\Var(f^{\leq d}_\delta) - 4\E_x[(f(x)-h(x))^2]}{4\log s}.\] 
\end{corollary} 

Consequently, as long as $\Var(f^{\leq d}_\delta) \ge 4\E_x[(f(x)-h(x))^2]+\eps$, we are guaranteed the existence of a variable with $\delta$-noisy influence at least 
\[ \Inf_i^{(\delta, d)}(f) \ge \frac{\eps}{4\log s}.\] 
%
%
\begin{proof}[Proof of~\Cref{cor:noisy-OSSS-truncated-agnostic}]
Applying~\Cref{thm:OSSS} with $h$ being the size-$s$ DT that is $OPT$ close to $f$, and $g$ being $f^{\leq d}_\delta$, we get that 
\begin{equation} \frac{1}{2}\Var(f^{\leq d}_\delta) - 2E[(h(x)-f^{\leq d}_{\delta}(x))^2] \le \Cov(h,f^{\leq d}_\delta) \le 2\sum_{i=1}^n \delta_i(h) \cdot \Inf_i(f^{\leq d}_\delta) \le  2\max_{i\in [n]}\Big\{ \Inf_i(f^{\leq d}_\delta)\Big\}\cdot \log s. \label{eq:apply-OSSS}
\end{equation} 
%
%
%
%
%\begin{align*}
%E[d(T(x), f^{\leq d}_{\delta}(x))] &= E[(T(x) - f^{\leq d}_{\delta}(x))^2]\\
%&\leq E[(T(x) - f(x))^2]+E[(f(x) - f_{\delta}(x))^2]+E[(f_{\delta}(x) - f^{\leq d}_{\delta}(x))^2]\\
%&\leq OPT+E[(f(x) - f_{\delta}(x))^2]+\epsilon\\
%&\leq OPT+\kappa+\epsilon
%\end{align*}
%
%
On the other hand, we also have that %
\begin{align*}
 \Inf_i(f^{\leq d}_\delta) &= \sum_{S \ni i, |S| \leq d} (1-\delta)^{2|S|} \wh{f}(S)^2  \tag*{(Formula for influence (\ref{eq:influence}))} \\
 &\le  \sum_{S \ni i, |S| \leq d} (1-\delta)^{|S|} \wh{f}(S)^2 \tag*{(since $(1-\delta)^{2k} \le (1-\delta)^{k}$ for all $k\ge 1$)}  \\
 &= \Inf^{(\delta, d)}_i(f).  \tag*{(Formula for $\delta$-noisy influence (\ref{eq:noisy-inf-fourier}))}
 \end{align*} 
 These two inequalities along with~\Cref{eq:apply-OSSS} give us 
 \[ \Var(f^{\leq d}_\delta) - 4\E_x(f(x)-h(x))^2 \le 4\max_{i\in [n]}\Big\{ \Inf_i^{(\delta, d)}(f)\Big\} \cdot \log s. \] 
 Rearranging completes the proof. 
\end{proof} 

\begin{fact}
$\Var(f_{\delta}) \leq \Var(f^{\leq d}_{\delta})+\epsilon$ for $d=\frac{\log(\frac{1}{\epsilon})}{\delta}$. 
\label{fact:truncated-variance}
\end{fact}

\begin{proof}
From formula for variance (\ref{eq:variance}), we know that 
$$\Var(f^{\leq d}_{\delta}) = \sum_{|S| \neq \emptyset, |S| \leq d} (1-\delta)^{2|S|}\hat{f}(S)^2$$
%
Also, 
\begin{align*}
\Var(f_{\delta}) &= \sum_{|S| \neq \emptyset} (1-\delta)^{2|S|}\hat{f}(S)^2   \\
&= \sum_{|S| \neq \emptyset, |S| \leq d} (1-\delta)^{2|S|}\hat{f}(S)^2 + \sum_{|S| \neq \emptyset, |S| > d} (1-\delta)^{2|S|}\hat{f}(S)^2\\
&\leq \Var(f^{\leq d}_{\delta}) + \sum_{|S| \neq \emptyset, |S| > d} e^{(-\delta)2|S|}\hat{f}(S)^2 \quad (\text{Using } 1+x \leq e^x)\\
&\leq \Var(f^{\leq d}_{\delta}) + e^{-2d\delta}\sum_{|S| \neq \emptyset, |S| > d} \hat{f}(S)^2 \quad (\text{Since } |S| > d)\\
&\leq \Var(f^{\leq d}_{\delta}) + e^{-2d\delta} \quad (\text{Since } \sum_{|S|}\hat{f}(S)^2 = 1)\\
&\leq \Var(f^{\leq d}_{\delta}) + \epsilon \quad (\text{Substituting the value of } d = \frac{\log(\frac{1}{\epsilon})}{\delta})
\end{align*}
\end{proof}
%
%
\begin{fact}
\label{fact:l2tol1}
For a boolean function $f:\pmo^n \to \pmo$, $\dist(f, \sign(\E[f])) \leq \E_x[(f(x)-c)^2]$ for any constant $c$.
\end{fact}
%
\begin{proof}
Let us assume that $f$ takes the value $1$ with probability $p$ and $-1$ with probability $1-p$ and without loss of generality, let us assume that $p \geq 0.5$. Now, $\dist(f, \sign(\E[f])) = \dist(f,1) = 2(1-p)$. We will prove the fact by showing that $\dist(f, \sign(\E[f])) \leq \min_c\E_x[(f(x)-c)^2]$.
$$\E_x[(f(x)-c)^2] = p(1-c)^2+(1-p)(1+c)^2$$
This quantity is minimized for the value $c = 2p-1$ and hence, we get that $\min_c\E_x[(f(x)-c)^2] = 4p(1-p)$. Now, we get the desired fact since $p \geq 0.5$ by assumption. 
%
\end{proof}
%
%
\begin{fact}
\label{fact:approx}
Let $T^{\circ}$ be a bare tree and let $T$ be the completion of the tree with respect to $f$ by putting $\sign(E[f_l])$ at each of the leaves $l$. Then, if $\sum_{\text{leaf} l \in T}2^{-l}\Var({(f^{\leq d}_l)}_{\delta}) \leq u$, then $\error_f(T) \leq 2u+2\epsilon + 8\kappa$
\end{fact}
%
%
\begin{proof}
From Fact \ref{fact:truncated-variance}, we know that if $\Var(f^{\leq d}_{\delta}) \leq u$, then $\Var(f_{\delta}) \leq u+\epsilon$. Therefore, we get that
%
$$\sum_{\text{leaf } l \in T}2^{-l}\Var((f_l)_{\delta}) = \sum_{\text{leaf } l \in T}2^{-l}E[((f_l)_{\delta} - E[(f_l)_{\delta}])^2]  \leq u+\epsilon$$
%
%Using the average noise sensitivity claim, we know that TODO(Prove average noise sensitivity claim)
From Fact~\ref{fact:stabilize-2}, we know that the average noise sensitivity of the functions $f_l$ obtained by restricting $f$ to the leaves of a tree $T$ is upper bounded by the noise sensitivity of the function $f$. Hence, we obtain that
%
\begin{align*}
\sum_{\text{leaf } l \in T}2^{-l}E[|{(f_l)}_{\delta}-f_{l}|] &\leq  2\kappa
\end{align*}
%
The factor of $2$ appears because noise sensitivity is defined in terms of probability of error and, since the range of functions if $[-1,1]$, the $\ell_1$ error is twice the probability of error. 
%

Since, the range of functions $f_l, (f_l)_{\delta}$ is $[-1,1]$, the $\ell_2$ error of the function is upper bounded by twice the $\ell_1$ error, hence
%
\begin{align*}
\sum_{\text{leaf } l \in T}2^{-l}E[({(f_l)}_{\delta}-f_{l})^2] &\leq 4\kappa
\end{align*}
%
Now, using $(a+b)^2 \leq 2(a^2+b^2)$, we get that
%
\begin{align*}
\sum_{\text{leaf } l \in T}2^{-l}E[(f_l-E[(f_{l})_{\delta}])^2] &\leq 2u+2\epsilon + 8\kappa
\end{align*}
%
Using Fact \ref{fact:l2tol1}, we get that
\begin{align*}
\error_f( T) = \sum_{\text{leaf } l \in T}2^{-l}\dist(f_l, \sign(\E[f_l])) \leq \sum_{\text{leaf } l \in T}2^{-l}E[(f_l-E[(f_{l})_{\delta}])^2] &\leq 2u+2\epsilon + 8\kappa
\end{align*}
%
\begin{comment}
Now, using Chebyshev's inequality, we know that 
$$Pr[|f_{\delta}(x)-E[f_{\delta}(x)]| \geq t] \leq \frac{\Var(f_{\delta})}{t^2}$$

Therefore, $Error(f_{\delta}, Ef_{\delta}) \leq t(1-\frac{\Var(f_{\delta})}{t^2}) + 2\frac{\Var{f_{\delta}}}{t^2} \leq t + 2\frac{\Var{f_{\delta}}}{t^2}$.

Now, if we consider the error of the completion of tree with respect to ${(f_l)}_{\delta}$ for each leaf $l$, we get that

\begin{align*}
\sum_{leaf l \in T}2^{-l}Error((f_{l})_\delta, T) &= \sum_{leaf l \in T}2^{-l}Error((f_{l})_\delta, E[(f_l)_{\delta}])\\
&\leq \sum_{leaf l \in T}2^{-l}( t + 2\frac{\Var{{(f_l)}_{\delta}}}{t^2})\\
&\leq t + \frac{2}{t^2}\sum_{leaf l \in T}2^{-l}\Var(f_{\delta})\\
&\leq t + \frac{4\epsilon}{t^2}
\end{align*}
%
For $t=\epsilon^{\frac{1}{3}}$, we get that 
%
\begin{align*}
\sum_{leaf l \in T}2^{-l}Error((f_{l})_\delta, T) &\leq 5\epsilon^{\frac{1}{3}}
\end{align*}
%
Using the average noise sensitivity claim, we get that TODO(Prove average noise sensitivity claim)
%
\begin{align*}
Error(f, T) = \sum_{leaf l \in T}2^{-l}Error(f_{l}, T) &\leq 5\epsilon^{\frac{1}{3}} + \kappa
\end{align*}
\end{comment}
\end{proof}
%
%
\subsection{Final argument (realizable)} 
\gray{

\textbf{todo: case split should be by whole tree, not leaf by leaf}
\begin{enumerate}
    \item $\Var((f_\ell)_\delta^{\le d}) \le \eps$ \textbf{todo: refer to notes}
    \item $\Var((f_\ell)_\delta^{\le d}) > \eps$.     Note that $\Stability_{\delta}(T,f) \le 1$ for any $T, f$, and when $T$ is the empty tree, $\Stability_{\delta}(T,f) = \Stab_{1 - 2\delta}(f)$. 


    
    Let $T_j$ be the partial tree of size $j$ that is build by the top-down algorithm. Let $\ell$ be the leaf split in the $j$-th iteration, and let $x_j$ be the variable it splits on. 

    \begin{definition}{Stability gain, restatement of \Cref{fact:stabilize-2}}
    $$SG(f, \ell, x_j) =  \frac{2\delta}{2^{|\ell|}}~\Inf_{x_j}^{1-2\delta}(f_{\ell })$$
    \end{definition}
    
    We claim the following: 
    \begin{claim}
    $$SG(f, \ell, x_j) \ge \frac{2\delta \eps}{j \log s}$$
    \end{claim}
    
    Consider the following sum: 
    \[\sum_{\ell \in T_j} SG(f, \ell, x_j) = \sum_{\ell \in T_j} \frac{2\delta}{2^{|\ell|}}~\Inf_{x_j}^{1-2\delta}(f_{\ell }) \]
    
    By \Cref{cor:noisy-OSSS-truncated}, there must be an index $i$ such that $\Inf_i^{(1-2\delta)}(f_\ell^{\leq d}) \ge \frac{\eps}{\log s}$. (\textbf{todo: we're assuming $\Var(f_\ell) \ge \eps$}). Note that $\Inf_i^{(1-2\delta)}(f_\ell) \ge \Inf_i^{(1-2\delta)}(f_\ell^{\leq d})$ for all $i$, since all Fourier coefficients in $f_\ell$ are at least as large as the corresponding coefficients in $f_\ell^{\le d}$. The algorithm chooses the variable which maximizes $\Inf_i^{(1-2\delta)}(f_\ell^{\leq d})$. Then splitting $\ell$ on $x_j$ yields the following stability gain: 
    
    \[SG(f, \ell, x_j) \ge \frac{2\delta \eps}{2^{|\ell|} \log s}\]
    
    Rewriting the sum: 
    \[\sum_{\ell \in T_j} SG(f, \ell) \ge \sum_{\ell \in T_j} \frac{2\delta \eps}{2^{|\ell|} \log s}\]
    \[\sum_{\ell \in T_j} SG(f, \ell) \ge \frac{2\delta \eps}{\log s} \sum_{\ell \in T_j} 2^{-|\ell|}\]
    \[\sum_{\ell \in T_j} SG(f, \ell) \ge \frac{2\delta \eps}{\log s}\]
    
    There are $j$ leaves, so by the pigeonhole principle, there must exist $\ell \in T_j$ such that $SG(f, \ell, x_j) \ge \frac{2\delta \eps}{j \log s}$. This is the leaf that we split on. \\
    
    Note that $\Stability_{\delta}(T,f) \le 1$ for any $T, f$, and when $T$ is the empty tree, $\Stability_{\delta}(T,f) = \Stab_{1 - 2\delta}(f)$. 
    
    So the size of the tree is the smallest size $t$ that satisfies
    
    \[\sum_{j = 1}^t \frac{2\delta \eps}{j \log s} \le 1 - \Stab_{1 - 2\delta}(f)\]
    \[\frac{2\delta \eps \log t}{\log s} \le 1 - \Stab_{1 - 2\delta}(f)\]
    
    
    \[t = O(s^\frac{1 - \Stab_{1 - 2\delta}(f))}{2\delta \eps})\]

\end{enumerate}
}
\subsection{Final argument (non-realizable)}
Let $f$ be such that $NS_\delta(f) \le \kappa$, let $h$ be a decision tree of size $s$ that is $\opt$-close to $f$ ($\opt = \E_x[(f(x)-h(x))^2]$). Let $T^\circ$ be a partial tree for $f$ built by {\sc BuildStabilizingDT}. We will bound the size of $T^\circ$ using the potential function argument from \Cref{fact:stabilize-2}. First we will restate this fact in terms of the change in the potential function when splitting a single leaf.

\begin{definition}{Stability gain, restatement of \Cref{fact:stabilize-2}}. \\

Let $T^\circ$ be a partial tree and ${T^\circ}'$ be this tree after splitting leaf $\ell$ on its maximally influential variable. Then we define the \emph{stability gain} of $\ell$:
    $$SG_\delta(f, \ell) = NS_\delta(T^\circ, f) - NS_\delta(T', f)$$
    $$SG_\delta(f, \ell) = \frac{\delta}{2^{|\ell|+1}(1-\delta)}\MaxInf^{(\delta)}(f_{\ell})$$
\end{definition}

$T^\circ$ must fall into one of the following cases:

\textbf{todo: change to $Var((f_\pi)_\delta$.}
\begin{enumerate}
    \item $\Ex_\pi [Var(f_\pi)] \le \opt + 2\kappa + 3\eps$: let $T^\circ_f$ be the $f$-completion of $T^\circ$, obtained by labeling the leaf of each path $\pi$ with $round(\Ex_x(f_\pi))$. By \Cref{fact:approx}, we have $\Ex_\pi [dist(f_\pi, (T^\circ_f)_\pi)] \le 2\opt + 4\eps + 5\kappa$.
    \begin{align*}
        \Pr_x[T^\circ_f(x) \ne f(x)] \textbf{todo: skip l2 distance, just use classification error}
    \end{align*}
    \item $\Ex_\pi [Var(f_\pi)_\delta] > 4\opt + \eps$:
    \begin{claim}
    \label{claim: score lower bound}
    There exists some path $\pi^*$ and variable $i^*$ such that 
    $$\frac{\Inf_{i^*}^\delta(f_{\pi^*})}{2^{|\pi^*|}} \ge \frac{\eps}{4|T^\circ| \log s}$$.
    \end{claim}
    Let $\MaxInf^\delta(f_\pi^{\le d})$ refer to $\max_{i \in [n]} [\Inf_i^\delta(f_\pi^{\le d})]$. We will use \Cref{cor:noisy-OSSS-truncated-agnostic} to lower-bound the average of this quantity over all paths $\pi$. 
    \begin{align*}
    \Ex_\pi [\MaxInf^{(1 - 2\delta)}(f_\pi^{\le d})] &\ge \frac{\Ex_\pi[Var((f_\pi)_\delta^{\le d}) - dist((f_\pi)_\delta^{\le d}, h_\pi)]}{\log s} \\
    &\ge \frac{\Ex_\pi[Var((f_\pi)_\delta^{\le d})] - \Ex_\pi[dist((f_\pi)_\delta^{\le d}, h_\pi)]]}{\log s}
    \end{align*}
    Note that $\Ex_\pi[dist((f_\pi)_\delta^{\le d}, h_\pi)] \le dist(f, h) + dist(f_\delta, f) + dist(f_\delta^{\le d}, f_\delta) \le \opt + \kappa + \eps$. Note also that $\Ex_\pi[Var((f_\pi)_\delta^{\le d})] \ge \Ex_\pi[Var((f_\pi)_\delta)] - \eps$ by \Cref{fact:truncated-variance}, and $\Ex_\pi[Var((f_\pi)_\delta)] \ge \Ex_\pi[Var(f_\pi)] - \Ex_\pi[NS_\delta(f_\pi)] \ge \Ex_\pi[Var(f_\pi)] - NS_\delta(f)]$. \textbf{todo: fix this, use proposition 9.1} Then $\Ex_\pi[Var((f_\pi)_\delta^{\le d})] \ge \Ex_\pi[Var((f_\pi)] - \kappa - \eps$.  \\
    

    \begin{align*}
    \Ex_\pi [\MaxInf^{(1 - 2\delta)}(f_\pi^{\le d})] &\ge \frac{\Ex_\pi[Var(f_\pi)] - (\opt + 2\kappa + 2\eps)}{\log s} \\
    &\ge \frac{\eps}{\log s}
    \end{align*}
    Put differently, we have 
    $$\sum_\pi \frac{\MaxInf^{(1 - 2\delta)}(f_{\pi^*})}{2^{|\pi|}} \ge \frac{\eps}{\log s}$$.
    The claim follows by pigeonhole principle.
\end{enumerate}

\Cref{claim: score lower bound} shows that as long as $\Ex_\pi [Var(f_\pi)] > \opt + 2\kappa + 3\eps$, then there exists a leaf of score at least $\frac{\eps}{|T^\circ| \log s}$, which {\sc BuildStabilizingDT} will split. Let ${T^{\circ}}'$ be the tree after splitting this leaf. By \Cref{fact:stabilize-2}:
\begin{align*}
    \Stability_\delta({T^{\circ}}', f) &= \Stability_\delta(T^\circ, f) + \frac{2\delta}{2^{|\pi^*|}} \cdot \Inf_{i^*}^{(1 - 2\delta) (f_{\pi^*})}\\
    & \ge  \Stability_\delta(T^\circ, f) + \frac{2\delta \eps}{|T^\circ| \log s}
\end{align*}
When $|T^\circ| = 0$, $\Stability(T^\circ, f)$ is simply $\Stab_{1 - 2\delta}(f) = 1 - 2\kappa$. When $|T^\circ| = t$, its maximum size, $\Stability(T^\circ, f)$ cannot be greater than 1. Then $t$ is at most the minimum $t$ that satisfies the following inequality: 
\begin{align*}
    \sum_{|T^\circ| = 1}^t \frac{2\delta \eps}{|T^\circ| \log s} &\le 1 - \Stab_{1 - 2\delta}(f) \\
    \frac{2\delta \eps \log t}{\log s} &\le 2\kappa\\
    t &= s^{O(\kappa/\delta\eps)}
\end{align*}
\textbf{todo: splits cannot increase variance.}

